Unraveling the Italian and English Telegram Conspiracy Spheres through Message Forwarding

Telegram has grown into a significant platform for news and information sharing, favored for its anonymity and minimal moderation. This openness, however, makes it vulnerable to misinformation and conspiracy theories. In this study, we explore the dynamics of conspiratorial narrative dissemination within Telegram, focusing on Italian and English landscapes. In particular, we leverage the mechanism of message forwarding within Telegram and collect two extensive datasets through snowball strategy. We adopt a network-based approach and build the Italian and English Telegram networks to reveal their respective communities. By employing topic modeling, we uncover distinct narratives and dynamics of misinformation spread. Results highlight differences between Italian and English conspiracy landscapes, with Italian discourse involving assorted conspiracy theories and alternative news sources intertwined with legitimate news sources, whereas English discourse is characterized by a more focused approach on specific narratives such as QAnon and political conspiracies. Finally, we show that our methodology exhibits robustness across initial seed selections, suggesting broader applicability. This study contributes to understanding information and misinformation spread on Italian and English Telegram ecosystems through the mechanism of message forwarding

==> 3-dataset.tex <==
\section{Designing and collecting the dataset}

\subsection{Preliminaries} 
Telegram is one of the most used messaging app, and is getting in the spotlight due to deplatforming, war in ucraine and war in the middle-east.\\
While there are a wide variety of chat types, such as gigachat and private, for this study we will focus our attenction on three:
\subsubsection{Channel}
Channels 



\subsection{Data collection} 
data e stats.

\begin{comment}
Platform Selection
The study focuses on Telegram due to its popularity among conspiracy theory groups for its privacy features and lack of content moderation compared to other social media platforms.

Time Frame
Data was collected from January 1, 2024, to mid-February 2024. This specific period was chosen to capture recent activities within these communities, allowing for an analysis of current trends and dynamics.


Types of Telegram Chats Analyzed
Personal Chats: Excluded from the study due to their private nature and lack of relevance to social network analysis.
Channels: Public or private broadcasts by admins to a passive audience, potentially with limited user comments.
Groups and Supergroups: Public or private groups allowing interactive discussions among members.
Gigagroups: Large-scale groups controlled by admins, without user comments.

The methodology likely involved using Telegram's API or third-party tools to scrape data from selected channels, groups, and supergroups. The focus was on extracting:

Messages: Content of communications within the groups.
Metadata: Information such as message timestamps, user IDs (anonymized), and chat IDs.
Group/Channel Metadata: Names, user counts, and descriptions.
User Interactions: Data on how members interact within these groups, including replies and mentions.
\end{comment}
